NodeReg: Mitigating the Imbalance and Distribution Shift Effects in Semi-Supervised Node Classification via Norm Consistency

Aggregating information from neighboring nodes benefits graph neural networks (GNNs) in semi-supervised node classification tasks. Nevertheless, this mechanism also renders nodes susceptible to the influence of their neighbors. For instance, this will occur when the neighboring nodes are imbalanced or the neighboring nodes contain noise, which can even affect the GNN's ability to generalize out of distribution. We find that ensuring the consistency of the norm for node representations can significantly reduce the impact of these two issues on GNNs. To this end, we propose a regularized optimization method called NodeReg that enforces the consistency of node representation norms. This method is simple but effective and satisfies Lipschitz continuity, thus facilitating stable optimization and significantly improving semi-supervised node classification performance under the above two scenarios. To illustrate, in the imbalance scenario, when training a GCN with an imbalance ratio of 0.1, NodeReg outperforms the most competitive baselines by 1.4%-25.9% in F1 score across five public datasets. Similarly, in the distribution shift scenario, NodeReg outperforms the most competitive baseline by 1.4%-3.1% in accuracy.

==> Sections/Acknowledgments.tex <==
\section{Acknowledgments}


==> Sections/Preliminary.tex <==
% \section{Related Work} \label{Sec-Pre&RelatedWork}
% \subsection{Graph Neural Network}\label{subsec-Graph_Neural_Network}
% Let $\mathcal{G}=\{\mathcal{V}, \mathcal{E}, \boldsymbol{X}\}$ denote a graph, where $\mathcal{V}$, $\mathcal{E}$ and ${\boldsymbol X}_v \in \mathbb {R}^{|\mathcal{V}|\times d_v}$ denote the sets of nodes, edges,  and the matrix of features of the nodes, respectively. For the representation $\mathbf{h}_v$ of node $v$, its propagation of the $k$-th layer GNN is represented as:
% % \begin{equation}\label{equa-gnns}
% % \begin{array}{cl}
% %    \mathbf{h}_v^{(k)}&=GNN(\mathbf{h}_v^{(k-1)};\theta)    \\
% %             &=\mathrm{UP}^{(k)}\big(\mathrm{AGG}^{(k)}\big( \mathbf{h}_u^{(k-1)}:\forall u \in \mathcal{N}(v)\cup v \big) \big) 
% % \end{array} 
% % \end{equation}
% \begin{equation}\label{equa-gnns}
% % \begin{array}{cl}
%    \mathbf{h}_v^{(k)} =\mathrm{UDT}^{(k)}\big(\mathrm{AGR}^{(k)}\big( \mathbf{h}_u^{(k-1)}:\forall u \in \mathcal{N}(v)\cup v \big) \big) 
% % \end{array} 
% \end{equation}
% where $\mathrm{AGR}(\cdot)$ denotes GNNs aggregate representations from the node $v$ with its neighbors $\mathcal{N}(v)$ and $\mathrm{UDT}(\cdot)$ denotes GNNs update the representation of node $v$ with trainable parameters. 

% We divide the set of nodes $\mathcal{V}$ on the graph $\mathcal{G}$ into a training set $\mathcal{V}_{train}$  (which includes a set of labeled nodes $\mathcal{V}_l$ with label set $\boldsymbol{Y} = \{y_1, y_2,...,y_l \}$ which is the label matrix for $c$ classes and a set of unlabeled nodes $\mathcal{V}_{u}$), a validation set $\mathcal{V}_{val}$, and a test set $\mathcal{V}_{test}$.


% \subsection{Problem Formulation}\label{subsec-Problem_Formulation}
% \subsubsection{Imbalanced Node Classification}\label{subsubSec-Problem-F-Imbalanced}
% We divide the set of nodes $\mathcal{V}$ on the graph $\mathcal{G}$ into a training set $\mathcal{V}_{train}$  (which includes a set of labeled nodes $\mathcal{V}_l$ with label set $\boldsymbol{Y} = \{y_1, y_2,...,y_l \}$ which is the label matrix for $c$ classes and a set of unlabeled nodes $\mathcal{V}_{u}$), a validation set $\mathcal{V}_{val}$, and a test set $\mathcal{V}_{test}$. The node imbalance classification problem refers to the situation where there is a significant discrepancy in the number of nodes from different classes within the $\mathcal{V}_{l}$, leading to poor classification performance for minority class nodes in the $\mathcal{V}_{u}$.

% \subsubsection{OOD Generalization on Graphs}\label{subsubSec-Problem-F-OOD}
% GNNs perform excellently in semi-supervised node classification on in-distribution data, i.e., test nodes generated from the same distribution as the training data. However, when the test data distribution shifts, GNNs often perform unsatisfactorily on OOD data.



